XRay: Enhancing the Web's Transparency with Differential Correlation

Today's Web services - such as Google, Amazon, and Facebook - leverage user data for varied purposes, including personalizing recommendations, targeting advertisements, and adjusting prices. At present, users have little insight into how their data is being used. Hence, they cannot make informed choices about the services they choose. To increase transparency, we developed XRay, the first fine-grained, robust, and scalable personal data tracking system for the Web. XRay predicts which data in an arbitrary Web account (such as emails, searches, or viewed products) is being used to target which outputs (such as ads, recommended products, or prices). XRay's core functions are service agnostic and easy to instantiate for new services, and they can track data within and across services. To make predictions independent of the audited service, XRay relies on the following insight: by comparing outputs from different accounts with similar, but not identical, subsets of data, one can pinpoint targeting through correlation. We show both theoretically, and through experiments on Gmail, Amazon, and YouTube, that XRay achieves high precision and recall by correlating data from a surprisingly small number of extra accounts.

==> archi/correlation.tex <==
\subsection{Differential Correlation}
\vspace{-3pt}
\label{s:correlation}

Targeting functions, which in this paper subsume advertising,
recommendations, and  personalization functions, are generally
complex and proprietary.  Approximating them will likely result
in fragile and service-specific designs.  Instead, our approach
is to disclose the result of personalization {\em when it occurs}:
recognize when particular a input has been chosen to trigger a
particular output.

For this, we build a series of inference models
that correlate the inputs to the outputs based on observations
from the user and shadow accounts.
% While our models are general,
% we describe their functionning in the context of a key simplifying
% assumption:  most targeted outputs result from a \emph{small} number
% of inputs, commonly a single one (an email or a product).
% \S\ref{s:extensions} extends those models to cover outputs that
% depend on larger combinations of inputs.
Overall, we design three types of inference models: one that detects
contextual targeting, one that detects behavioral targeting, and
one that combines the two to detect both. After formalizing the
problem, we describe each model in turn.

\heading{Assumptions and Problem Formulation.}
\xray abstracts Web targeting as a black box function $f$ that represents a
service (\eg Gmail) associating inputs $D_i$s (\eg the emails received
and sent) to targeted outputs $O_k$s (\eg ads). 
combinations...
Other inputs are either ignored
by \xray, known only to targeting system, or under no known control. \xray
assumes they are independent or fixed, captured in the randomness of $f$.
Assumptions about $f$, and the range of functions \xray supports, are discussed
further in \S\ref{s:assumptions}.
Our goal is to decide separately for each output $O_k$ whether $f$ produced it
as a reaction to one of the $D_i$s (an event denoted by $D_i$), or whether $O_k$
is untargeted (an event we denote by $D_\emptyset$).
Differential Correlation uses two main techniques to detect this correlation: set
intersection and Bayesian inference.

\heading{Behavioral Targeting With Set Intersection.}
Intuitively, Differential Correlation leverages observations $x_i$, which are
outputs observed in shadow accounts.  From these observations
and for a given output $O$, \xray constructs the set of accounts in which
$O$ was observed, that we call the {\em Active Accounts}.
Given that outputs will appear more often in accounts containing the targeting
inputs, the core of the algorithm is to collect the inputs appearing
in most Active Accounts.

For a given output (\eg an Ad), we thus intersect the sets of
inputs present in each Active Account. This intersection is the combination of
emails that most likely explains the output's presence.
Note that we need to take noise into account: an ad might appear in an account
that doesn't have the right emails. We take this into account by requiring the
emails to be in a large fraction, but not necessarily all, of the Active
Accounts.
This is step 2 in the full algorithm described in \F\ref{f:algo}.

The algorithm performs four other steps to improve accuracy and use shadow
accounts more efficiently. First, we need enough Active Accounts to be
reasonably sure of our targeting correlation. In step 1 we make sure we have
enough data to conclude, and return non targeted if we don't have enough Active
Accounts.
Second, it is unlikely that a significant fraction of the Inactive Accounts
contain the targeting combination. We use this information in step 3 and filter
out emails that are in too many inactive accounts.
Third, our algorithm only detects bounded combinations with good accuracy as we
will develop in \S\ref{s:assumptions}. In step 4, we make sure we don't predict
too big combinations.
Finally, in step 5 we make sure we detect real combinations: the whole
combination should be contained in a significant fraction of the Active
Accounts, and not just subsets of it.

\begin{figure}[t]
% \vspace{-0.3cm}
\centering
\begin{lstlisting}[mathescape]
data = an output (e.g. an Ad)
params = threshold, min_active_accs, max_combination_size
Active Accounts (AA) = the accounts that see the Ad
// Step 1: enough data?
if nb of AA < min_active_accs:
  return $\emptyset$
// Step 2: select emails in most AA
results = email(s) in the maximum number of AA
if $\frac{results~size}{AA~size} < threshold$:
  return $\emptyset$
// Step 3: penalize low coverage
results = email(s) from results in minimum number of
     Inactive Accounts
// Step 4: bounded combination size?
if results size > max_combination_size:
  return $\emptyset$
//Step 5: verify it is a real combination
if results size > 1
 and $\frac{number~of~AA~containing~all~results}{AA~size} < threshold$:
  return $\emptyset$
// results is now the predicted targeting
return results
\end{lstlisting}
\vspace{-0.4cm}
\caption{Behavioral targeting detection with Set Intersection.}
\label{f:algo}
\end{figure}

\heading{Behavioral Targeting With Bayesian Inference.}
The Set Intersection algorithm we just described gives a great intuition of
our inference process. However it makes early decisions and requires parameters
tuning.
In the prototype, we thus use a Bayesian Inference algorithm that leverages the
same information and gives very similar accuracy. The advantages is that the
Bayesian model is more robust to noise and parameters can be automatically
learned by iterated inference.

The Bayesian correlation model defines observations as a simple binary signal
per account, $x_j=1$ if the ad were observed in account $j$ and $0$ otherwise.
We define three probabilities. First, the {\em coverage} $\pin$ is
the probability that an account $j$ with the explaining input $D_i$ sees the
explained output at least once.
Second, an account $j'$ without input $D_i$ would see the ad with a smaller
probability $\pout$. $\pout$ acts like the threshold of the previous algorithm:
the smaller it is, the more we penalize seeing the output without the input.
Third, if the ad is not behaviorally targeted, it will appear in each account with
the same probability $\punt$.
If we define $A_x$ to be the set of accounts that have seen the ad, and $A_i$
the set of accounts that contains email $D_i$, then we have:
\[
\begin{disarray}[c]{rl}
\small
	\probaof{\vec{x}\cond D_i} 
	= &
	\left( \pin\right)^{|A_x|} \left( 1-\pout \right)^{|\bar{A_x}|}  \\ & \times
	\left(\frac{1-\pin}{1-\pout}\right)
	 ^{|A_i \cap \bar{A_x}|} 
	 \left(\frac{\pout}{\pin} \right)
	^{|\bar{A_i}\cap A_x|}
	 \\
	
\probaof{\vec{x}\cond D_\emptyset} = & 
\left( \punt \right)^{|A_x|} 
\left(1- \punt \right)^{|\bar{A_x}|}
\ff
\end{disarray}
\]
These scores are then normalized and give the probability of every input to explain
a given output. We can then chose the highest score.

\heading{Contextual Targeting.}
Contextual targeting is more straight forward since it uses content
shown immediately next to the ad.
\xray also uses Bayesian Inference, and defines the observations as how many
times ad $O_k$ is seen next to email $D_i$.
Our causal model assumes imperfect coverage: if
this ad is contextually targeted towards $D_i$, it will occur next to this email
with probability $\pin<1$ and next to any other email with probability $\pout$.
Alternatively, if the ad is untargeted, our model predicts it will be shown
next to any email with probability $\punt$. Hence, \(
\probaof{\vec{x}\cond\!\! D_i}  = \left( \pin \right)^{x_i} \left( \pout \right)^{\sum_{i'\neq i} x_i'},
\probaof{\vec{x}\cond\!\! D_\emptyset}  = \left( \punt \right)^{\sum_{i} x_i}
\).
For this model, parameters are also automatically computed by iterated inference.

\heading{Composite Model (\xray).}
The preceding contextual and behavioral mechanisms are designed to detect
different types of targeting. To detect both, \xray combines them into a
{\em composite model}, which averages scores from individual models.
Our experimental results, described in \S\ref{s:eval:accuracy}, demonstrate
that doing so yields higher recall for no loss in precision.

While contextual targeting can reuse observations from the same account by
simply reloading the page or loading a different email, behavioral targeting
requires multiple accounts to gather multiple points of observation. We next
describe \xray's strategy to minimize the number of accounts needed.











\iffalse
Targeting functions, which in this paper subsume advertising,
recommendations, and  personalization functions, are generally
complex and proprietary.  Approximating them will likely result in fragile and
service-specific designs.  Instead, our approach is to disclose
the result of personalization {\em when it occurs}:  recognize
when particular input has been chosen to trigger a particular
output.  For this, we build a series of Bayesian inference models
that correlate the inputs to the outputs based on observations
from the user and shadow accounts.  While our models are general,
we describe their functioning in the context of a key simplifying
assumption:  most targeted outputs result from a \emph{small} number
of inputs, commonly a single one (an email or a product).
\S\ref{s:extensions} extends those models to cover outputs that
depend on larger combinations of inputs.

Overall, we design three types of inference models: one that detects
contextual targeting, one that detects behavioral targeting, and
one that combines the two to detect both. After formalizing the
problem, we describe each model in turn.


\heading{Assumptions and Problem Formulation.}
\xray abstracts Web targeting as a black box function $f$ that represents a
service (\eg Gmail) associating tracked inputs $D_i$s (\eg the emails received
and sent by a user) to targeted outputs $O_k$s (\eg ads). Other inputs are
either ignored by \xray, known only to targeting system, or under no known
control (variables $R_j$). \xray assumes they are independent or fixed, captured
in the randomness of $f$.
Our goal is to decide separately for each output $O_k$ whether $f$ produced it
as a reaction to one of the $D_i$s (an event denoted by $D_i$), or whether $O_k$
is untargeted (an event we denote by $\emptyset$).

Intuitively, Differential Correlation is a simple generative model to simulate
the audited service, given some targeting associations (\eg $D_a$ triggers
$O_b$). We then compute the probability for this model to generate the outputs
we do observe, for every targeting association. The most likely association will
be the one \xray returns.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{figures/PriorPosterior.pdf}
	\end{center}
    \vspace{-10pt}
    \caption{{\bf Overview of Differential Correlation.} 
    \vspace{-10pt}
}
	\label{f:priorposterior}
\end{figure}
More precisely, differential correlation holds an initial belief about the
plausibility of each possible association, denoted
$\vec{\pi}=(\pi_1,\pi_2,\ldots,\pi_N,\pi_\emptyset)$\footnote{Since all inputs
  $D_i$s play a similar role, we can set $\pi_i=\pi_{i'}$. The value of
  $\pi_{\emptyset}$ can be adapted depending on the domain~(\eg it was reported
  that half of all Websites have less than 20\% of untargeted ads). In practice
  having equal probability $\pi_i=\pi_\emptyset=\frac{1}{N+1}$ has been 
robust.}. It then uses new observations created by \xray's multiple accounts
to update this probability into a posterior belief $\vec{\hat{\pi}}$. Typically,
observations reinforce likeliness for one of the events, so this posterior has a
higher maximum coefficient.

As shown in Fig.\ref{f:priorposterior}, the new belief is obtained after: (1)
specifying the observations, (2) defining a causal model, and (3) (not shown)
applying Bayes' rule.
\[	
\hat{\pi}_i
%=\probaof{D_i \cond \pi, \vec{x}} 
= \frac{\probaof{\vec{x} \cond D_i} \times \pi_i}{C}
\midwor{and}
\hat{\pi}_\emptyset
%=\probaof{D_\emptyset \cond \pi, \vec{x}} 
= \frac{\probaof{\vec{x} \cond D_\emptyset} \times \pi_\emptyset}{C}
				\vf
\]
where $C=\sum_{i=1}^N{\probaof{\vec{x} \cond D_i} \pi_i}+\probaof{\vec{x} \cond D_\emptyset} \pi_\emptyset$ is a normalizing constant such that the probability vector $\vec{\hat{\pi}}$ has unit sum.



% \heading{How to update our belief with observations?}
% Three steps are required and done by \xray: (1) Define the observations; (2) Define the causal model; (3) Apply Bayes' rule. Each of these step in general depends on what kind of targeting \xray is currently inferring; for the targeting we analyze they usually resemble one of three model. We will present first how these steps operate for \emph{contextual targeting}.
% 
% \begin{enumerate}
% 	\item Define the observations: The \xray system runs a series of monitoring test and observe specific outputs with varying inputs. For each output $O_k$ we first synthesize these data into a vector $\vec{x}$ of $M$ values: Observations could be quantitative (\eg ``How many times did we observe this ad when email $i$ was shown?'') or binary (\eg ``Was this ad shown at least once to account $j$?''). Each may correspond to a particular email (\ie $M=N$ and $\vec{x}=(x_1,\ldots,x_N)$) or to a particular account.
% 	\item Define the causal model: We assume that no matter how complex the targeting is, its behavior with regard to inputs remains relatively simple. More formally, for each output $O_k$ we assume that it could be one of two cases: First, it may be that $O_k$ is untargeted (\ie the event we denote by $\emptyset$). The same probability model can then be used to explain all values of $\vec{x}$ independently of their index that represent different inputs. Second, it could also be that this output $O_k$ is targeted at a particular input $D_i$, in which case we should expect the likeliness of an observation $\vec{x}_j$ to heavily depend on whether $j$ and $i$ are related.
% \(	
% \hat{\pi}_i
% %=\probaof{D_i \cond \pi, \vec{x}} 
% = \frac{\probaof{\vec{x} \cond D_i}}{\sum_{i=0}^N \probaof{\vec{x} \cond D_i}}
% 				\vf
% 				\) where with a slight abuse notation we denote $D_\emptyset$ by $D_{0}$ and $\hat{\pi}_\emptyset=\hat{\pi}_{0}$.
% \end{enumerate}



\heading{Contextual Targeting.} 
Given that targeting uses the content shown immediately next to the ad,
\xray defines the observations as how many times ad $O_k$ was seen when the
email $D_i$ is shown. Our causal model assumes imperfect \emph{coverage}: if
this ad were contextually targeted towards $D_i$, it would occur next to this email
with probability $\pin<1$ and next to any other email with probability $\pout$.
Alternatively, if the ad were untargeted, our model predicts it would be shown
next to any email with probability $\punt$. Hence, \(
%\begin{disarray}[c]{rl}
\probaof{\vec{x}\cond\!\! D_i}  = \left( \pin \right)^{x_i} \left( \pout \right)^{\sum_{i'\neq i} x_i'}, %\\
\probaof{\vec{x}\cond\!\! D_\emptyset}  = \left( \punt \right)^{\sum_{i} x_i}
%\end{disarray}
\)
How should parameters $\pin,\pout,\punt$ be chosen in this model?  We expect
$\pin>\punt$ since a targeted ad is shown more often. Similarly $\pout$ is
expected to be the smallest since a targeted ad is by definition not shown
outside its appropriate context. \xray automatically infers these parameters
values using iterated inference (\eg in a representative Gmail experiment,
$(\pin,\pout,\punt)$ converged to $(0.58,0.04,0.10)$). Details are omitted for
space reasons.

\heading{Behavioral Targeting.} Behavioral targeting is more challenging to
detect since each ad could be related to various emails in the account. The
differential correlation model defines observations as a simple binary signal
per account, $x_j=1$ if the ad were observed in account $j$ and $0$ otherwise.
Both values are considered useful information. Our causal model resembles the
one above: if the ad were targeted towards $D_i$, then an account $j$ containing
$D_i$ would see this ad at least once with a \emph{coverage} probability $\pin$,
or otherwise would miss it with probability $(1-\pin)$. An account
$j'$ without input $D_i$ would see the ad with a smaller probability $\pout$, missing
it with probability $(1-\pout)$. If the ad were not behaviorally
targeted, it would appear in each account with the same probability $\punt$. 
% In summary we have:
% \[
% \begin{disarray}[c]{rl}
% 	\probaof{\vec{x}\cond D_i} = & 
% 	 \left( \pin \right)^{\sum_{j|\; i\in J} x_j} 
% 	\left(1- \pin \right)^{\sum_{j|\; i\in J} (1-x_j)} \\ & 
% 	\times
% 	\left( \pout \right)^{\sum_{j|\; i\notin j} x_j}
% 	\left(1- \pout \right)^{\sum_{j|\; i\notin j} (1-x_j)}
% 	 \\
% \probaof{\vec{x}\cond D_\emptyset} = & 
% \left( \punt \right)^{\sum_{j} x_j}
% \left(1- \punt \right)^{\sum_{j} (1-x_j)}
% \ff
% \end{disarray}
% \]
If we define $A_x$% = \lset j \dimset x_j=1 \rset$ 
to be the set of accounts that have seen the ad, and $A_i$ the set of accounts that contains email $D_i$, then we have:
\[
\begin{disarray}[c]{rl}
	\probaof{\vec{x}\cond D_i} 
% 	= & 
% 	 \left( \pin \right)^{|A_i\cap A_x|} 
% 	 \left(1- \pin \right)^{|A_i \cap \bar{A_x}|} \\ & 
% 	\times
% 	\left( \pout \right)^{|\bar{A_i}\cap A_x|}
% 	\left(1- \pout \right)^{|\bar{A_i}\cap \bar{A_x}|}
% 	\vf \\ 
	= &
	\left( \pin\right)^{|A_x|} \left( 1-\pout \right)^{|\bar{A_x}|}  \\ & \times
	\left(\frac{1-\pin}{1-\pout}\right)
	 ^{|A_i \cap \bar{A_x}|} 
	 \left(\frac{\pout}{\pin} \right)
	^{|\bar{A_i}\cap A_x|}
	 \\
	
\probaof{\vec{x}\cond D_\emptyset} = & 
\left( \punt \right)^{|A_x|} 
\left(1- \punt \right)^{|\bar{A_x}|}
\ff
\end{disarray}
\]
This form allows easy interpretation. From the point of view of the event $D_i$,
an account found in $A_i \cap \bar{A_x}$ plays the role of a false positive (an
ad was expected when it was not shown). This should penalize our belief
$\hat{\pi}_i$, especially when the \emph{coverage} $\pin$ is close to $1$.
Inversely, an account found in $\bar{A_i}\cap A_x$ is a false negative (we
observed an ad where we did not expect it), which should decrease probability
$\hat{\pi}_i$, especially when $\pout$ is close to $0$.

\heading{Composite Model (\xray).}
The preceding contextual and behavioral mechanisms are designed to detect
different types of targeting. To detect both, \xray combines them into a
{\em composite model}, which averages scores from individual models.
Our experimental results, described in \S\ref{s:eval:accuracy}, demonstrate
that doing so yields higher recall for no loss in precision.

\fi


==> archi/placement.tex <==
\subsection{Input Placement}
\vspace{-3pt}
\label{s:placement}

Our algorithm to infer behavioral targeting computes the most likely input from
a set containing $N$ items that explains a particular set of observations
$\vec{x}$ obtained by \xray. It raises an immediate question: how should we
place emails in shadow accounts, and how many shadow accounts do we need in
order to correctly detect targeting from the observations?  We build up to our
answer, which surprised us.
% under which conditions on the number of accounts used and the placement of emails in the shadow accounts can we expect this observations to reveal the correct targeting?

\heading{First Try: Exponential.}
A first na\"ive but certainly comprehensive answer is to create accounts for
every combination of inputs, gathering maximum information about their
behaviors. As long as $\pin>\punt>\pout$, one could expect with a sufficient
number of observations to detect which accounts, and hence which subsets of
inputs, target a particular ad. Unfortunately, this method requires a number of
accounts that grows \emph{exponentially} as the number of items $N$ to track
grows.

\heading{Second Try: Linear.}
If we believe, as our experiments validated, that many targeted ads are
explained by a \emph{single} input, then an alternative method is to create one
account for each possible input (\eg the account has only one input, or all inputs
but one).
The method of correlation could then resemble the one we presented for
contextual targeting, with $N$ points of observation: with sufficient
observations, for any value $\pin>\punt>\pout$, only the targeted inputs will
generate associations for a given ad.
% This strategy suffers from three main problems. First it has no chance to detect
% targeting by combinations of emails. Second, because of low coverage, this strategy
% will miss many ads. Third,
Maintaining a {\em linear} number of accounts in the number $N$ of inputs is an
improvement over the first try. However, it remains impractical to scale to
large input sizes (e.g., a mailbox).

\heading{Result: Logarithmic.}
We now show that it is possible to obtain guaranteed answers to infer behavioral
targeting using no more than a \emph{logarithmic} number of accounts as a
function of the number of inputs. The key insight is that combining multiple
inputs inside one account provides extra information that can be combined to
inform the inference. Intuitively, a logarithmic number of observations provides
$\log(N)$ bits, which is the appropriate order to choose correctly an element in
a set of $N$ hypotheses.  Interestingly, while our initial placement and
decision algorithms were deterministic mechanisms based on encoding, we
substantially simplified the design to obtain a more robust {\em randomized}
algorithm. Our final assignment is to pick a probability $0<\alpha<1$
and fill each account randomly such that any input $i$ is included
with probability $\alpha$.

\begin{thm}
	Assuming that $\pin,\punt$ are fixed and $\pout$ is strictly smaller than $\pin$
  (bounded noise hypothesis)
  % and $\pout=0$
  , then for any $\varepsilon$ there exists an algorithm using $C \times \ln(N)$ accounts that correctly identifies the inputs of a targeted ad with probability $(1-\varepsilon)$.
	\label{res:placement}
\end{thm}

The gist of the proof is to show that the algorithm from \F \ref{f:algo} is
asymptotically correct with the random placement we just described.
Let us call C the set of inputs contained in a {\em significant fraction} of
the Active Accounts. If there is no targeting, then these inputs are present
in the accounts by mere chance, and we can show using Chernoff bounds that
the probability of C not being empty decreases exponentially fast with the
number of active accounts. If there is targeting, because of the bounded noise
hypothesis, and using Chernoff bounds again, we can show that with high probability
no other input than the explaining combination is in C. The full proof is described
in Appendix~\ref{s:correctnessproof}.

% First, pick a probability $0<\alpha<1$. Second, create $C\times
% \log(N)$ accounts and fill each randomly such that any input $i$ is included
% with probability $\alpha$. Third, run a number of observations and compute for
% each output $O_k$ the set of \emph{active} accounts as those that see the
% output. Define the set of \emph{core} inputs, $S(O_k)$, as those appearing in
% \emph{all} active accounts. Finally, return the following results: if
% $S(O_k)=\{D_i\}$, associate $O_k$ with input $D_i$, otherwise return $\emptyset$
% to denote that this ad is untargeted. We prove correctness in a more general
% case in Appendix~\ref{s:correctnessproof}. 


% \[
% \left\{
% \begin{disarray}[c]{ll}
% 	\midwor{if} S(O_k) = \emptyset, & \midwor{\texttt{return} ``untargeted'',} \\
% 	\midwor{if} S(O_k) = \lset D_i \rset, & \midwor{\texttt{return} ``targeted by $D_i$'',}  \\
% 	\midwor{if} |S(O_k)| \geq 2, & \midwor{\texttt{return} ``undefined''.} \\
% \end{disarray}
% \right.
% \]

%See Appendix A for a formal proof.  
%Interestingly, the proof does not require that $\pin>\punt$.

% First is the claim that any untargeted ads will end up with probability $(1-\varepsilon)$ with an empty core subset. This occurs because this ad is shown on an expected number of $C\times \log(N) \times\punt$ accounts chosen randomly. The probability that an input appears in all of them vanishes as $N$ goes large. Second is the claim that any ad targeted towards $D_i$ has with probability $(1-\varepsilon)$ a singleton core subset equal to $\{D_i\}$. It is immediate, since $\pout=0$, that all active accounts for this ad contain $D_i$. In fact, $C\times \log(N) \times \alpha \times \pin$ such active accounts exist in expectation. By the same argument as above, the probability that another email is present by chance in all of them vanishes as $N$ goes large. See Appendix A for a formal proof of both claims.  Interestingly, the proof does not require that $\pin>\punt$.



==> architecture.tex <==
\vspace{-10pt}
\section{The \sysname\ Architecture}
\vspace{-10pt}
\label{s:architecture}

% Shorter
\xray's design addresses the preceding goals. For
concreteness, we draw examples from our three \xray instantiations: tracking
email-to-ad targeting association within Gmail, attributing recommended videos
to those already seen on YouTube, and identifying products in the
wish list that generate a recommendation on Amazon.

%We next describe our \xray design, which addresses the preceding goals.  Although \xray is generally applicable to many Web services and use cases, we use examples from our Gmail, YouTube, and Amazon experience.  On Gmail, we track email-to-ad associations; on YouTube, we explain why certain videos are recommended to users based on the videos they viewed previously; and on Amazon, we explain which products are recommended to users based on the contents of their carts and wish lists.

\subsection{Architectural Overview}
\label{s:overview}

\F\ref{f:architecture} shows \xray's high-level architecture, which consists of
three components: (1) a {\em Browser Plugin}, which intercepts tracked inputs
and outputs to/from an audited Web service and provides users with visual
feedback about any input/output associations; (2) a {\em Shadow Account
Manager}, which populates the shadow accounts with inputs from the plugin and
collects outputs (e.g., ads) for each shadow account; and (3) the {\em
Correlation Engine}, \xray's core, which infers associations and provides them to
the plugin for visualization.  While the Browser Plugin and Shadow Account
Manager are {\em service specific}, the Correlation Engine, which encapsulates
the science of Web-data tracking, is {\em service agnostic}.  For example,
implementing the plugin and shadow account managers for Gmail, Amazon, and
YouTube was conceptually simple and only took about 500 lines of code per
service; zero changes were needed in the correlation engine.  After we describe
each component in turn, we focus on the design of the correlation engine.

The {\bf Browser Plugin} intercepts designated inputs and outputs (i.e., {\em tracked
inputs/outputs}) by recognizing specific DOM elements in an audited service's
Web pages.  Other inputs and outputs may exist that \xray does not track
(i.e., {\em untracked inputs/outputs}).  The decision of what to track belongs to an investigator or developer who instantiates
\xray to work on a specific service. For example, in the \xray Gmail plugin, we
configured \xray to monitor a user's emails as inputs and ads as outputs.
When the plugin gets a new tracked input (e.g., a new email), it allows it
to go to the service but also forwards it to the shadow account
manager.
When the plugin gets a new tracked output (e.g., an ad), it queries the
correlation engine for associations with the user's tracked inputs (message
{\code get\_assoc}).
% It displays any associations returned to the user.
% \F\ref{f:screenshot} shows a specific visualization of associations
% that we implemented for our Gmail \xray plugin.  It shows above each ad a
% colored label indicating whether the ad is targeted; clicking on a targeted
% label shows which email(s) triggered the ad.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/architecture}
\caption{\small {\bf The \xray Architecture.}
}
\label{f:architecture}
\vspace{-0.1cm}
\end{figure}


The {\bf Shadow Account Manager} is responsible for: (1) populating the shadow
accounts with subsets of a user account's tracked inputs, and (2) periodically
retrieving outputs from the audited service for each shadow account.  Both
functions are service specific.  For Gmail, they involve sending emails with
SMTP and invoking the ad API to request ads.  For YouTube, they involve
streaming a video and scraping recommendations, and for Amazon, they involve
placing products in wish lists and scraping recommendations.  The complexity of
these tasks depends on the availability of APIs or the stability of a service's
page formats.  Outputs collected from the Web service are placed into a {\em
Correlation Database}, which maps shadow accounts to their input sets and output
observations.  \F\ref{f:architecture} shows a particular assignment of tracked
inputs across three shadow accounts. For example, Shadow 1 has inputs $D1$ and
$D2$.  The figure also shows the outputs collected for each of the shadow
accounts.  Output $O1$ appears in Shadows 1 and 2 but not in Shadow 3; output
$O2$ appears in Shadow 3 only.

The {\bf Correlation Engine}, \xray's service-agnostic ``brain,'' leverages the
data collected in the correlation database to infer input/output associations.
Three key functions ensure that associations can be best inferred under
stringent shadow account constraints:  First, the {\em Differential Correlation}
module performs Bayesian inference to detect associations,
incrementally leveraging new output observations. Second, the {\em Input Placement} module
distributes tracked inputs across shadow accounts.  Third, the
{\em Input Matching} lets \xray use shadow accounts to maximum
advantage by reducing overlaps between distributed inputs.

Conceptually, the correlation engine works as follows.  When new outputs from
shadow accounts are added into the correlation database, the engine
attempts to diagnose each output using the {\em Differential Correlation}
module (\S\ref{s:correlation}). In \F\ref{f:architecture}, it might conclude that
$D2$ triggers $O1$ (denoted $D2 \rightarrow O1$) because $O1$ appears
consistently in accounts with that $D2$. It might also conclude that $O2$ is
{\em untargeted} given inconsistent observations.  The
engine saves these associations in the correlation database.
When the plugin makes a {\code get\_assoc} request, the engine
looks up the specified output in its database and returns any association.
If the output is not found, then the engine replies  {\em unknown}.  For
example, if an ad never appeared in any shadow account,
\xray is unable to explain it.  Periodic data collection, coupled with
an online update of correlation model parameters, minimizes the number of
unknown associations.  In our Gmail experience, collecting shadow account
outputs every ten hours or so yielded few unknown ads.

The above example is overly simplistic, and \xray handles several key challenges
occurring in practice.  First, outputs are never consistently
seen across all shadow accounts containing the input they target. We call
this the {\em limited-coverage} problem; \xray's input placement
module (described in \S\ref{s:placement}) handles it by placing each data input
in more shadow accounts.  Perhaps surprisingly, we show that under realistic
assumptions, the required number of accounts grows logarithmically in the number
of inputs, where the log's constant depends on the coverage (low coverage means
a higher constant).  \S\ref{s:eval:scalability} validates this theoretical
result with experiments on Gmail, Amazon, and YouTube.

% \iffalse As new outputs from the shadow accounts are added into the correlation
% database, the engine attempts to associate them to any inputs, saving any
% associations in a separate table in the correlation database.  When the plugin
% makes a {\code get\_assoc} request, the engine looks up the specified output and
% returns any association, or {\em unknown} if the output is not found (\eg a
% brand new ad that has not yet been observed). Periodic data collection, coupled
% with an online update of correlation model parameters, minimizes the number of
% unknown associations. In our Gmail experience, collecting shadow account outputs
% every ten hours or so yielded few unknown ads.

% \heading{Correlation Engine Modules.} Before detailing the correlation engine's
% three modules, in the remainder of this section, we describe the fundamental
% technical challenges they address.  Identifying targeting requires to jointly
% consider output observations. For instance, in \F\ref{f:architecture}, one
% concludes that $D2$ likely triggers $O1$ because $O1$ consistently appears in
% accounts that includes $D2$ three times. In contrast, $O2$ provides more support
% for being \emph{untargeted}, as no single input seems to be consistently
% associated with it. \emph{Differential correlation} (\S\ref{s:correlation})
% introduces a simple and effective probabilistic model of the two most prevalent
% forms of targeting.  Parameters of our model can be refined in real time in an
% unsupervised manner. 

% The above example is overly simplistic, and \xray handles two critical
% challenges occurring in practice.  First, outputs are never consistently seen
% across all shadow accounts containing the input they target. We call this the
% {\em limited-coverage} problem; \xray's {\em input placement} module (described
% in \S\ref{s:placement}) handles it by placing each data input in more shadow
% accounts.  Perhaps surprisingly, we show that under realistic assumptions, the
% required number of accounts grows logarithmically in the number of inputs, where
% the log's constant depends on the coverage (low coverage means a higher
% constant).  \S\ref{s:eval:scalability} validates this theoretical result with
% experiments on Gmail, Amazon, and YouTube.

% \fi

%What complicates this analysis is that outputs are not deterministically seen across all shadow accounts containing the input they target, a problem we call the {\em limited-coverage} problem. Our targeting model explicitly accounts for this, and our input placement (see below) replicates on purpose each input in various shadow accounts. 

%One of the correlation engine's powers is that it can be deployed to arbitrary input sets of interest, but that typically raises a \emph{scalability} issue. It seems that only so much can be tracked when shadow accounts are a costly resource that should be minimized.  Perhaps surprisingly, we show that the required number of accounts grows \emph{logarithmically} in the number of inputs when a simple \emph{randomized placement} is used (\S\ref{s:placement}). XX Scaling the probability XX also addresses limited coverage. We show experimentally that \xray applied to Gmail, Amazon, and YouTube exhibits scalability remarkably similar to our prediction. 

Second, an output may have been triggered by one of several targeted inputs (\eg
multiple emails on the same topic may cause related ads to appear), a problem we
refer to as \emph{overlapping-inputs}. This at best exacerbates the number of
accounts needed, as it roughly diminishes the differential signal we receive
among them. Grouping inputs \emph{a priori} seems to contradict our stated goal
not to depend on their content. Remarkably, \xray's {\em input matching} module
(see~\S\ref{s:input_matching}) leverages partial observation from the outputs
and succeed in matching overlapping inputs, a result we also empirically
validate. This boosts differential signals and hence \xray's efficiency.


%Third, untracked inputs could potentially disrupt our ability to detect correlations for tracked inputs.  While we generally ignore these inputs, we try to preserve constant across the shadow accounts the IP addresses and basic profile information, such as sex, age, or zip code.  These inputs are often used in combination with other inputs, such as emails, to target ads.  If an untracked input is replicated across shadow accounts, any ads targeted against that input will appear in many diverse accounts, and \xray will declare those ads untargeted.  If an untracked input is not replicated across shadow accounts, any ads targeted against it will be missing from all shadows, causing \xray to return an unknown association.

% \heading{Organization.}
% The remainder of this section provides further detail on the design
% of the correlation engine, \xray's ``brain.''  After briefly reviewing how
% targeting works today (\S\ref{s:background}), we examine the correlation
% engine's modules: differential  correlation , input
% placement (\S\ref{s:placement}), and input matching (\S\ref{s:input_matching}).

All these modules are service agnostic, entirely novel in either their design or
analysis, and a significant value-added benefit for an auditor or a developer to
build auditing tools atop \xray. We therefore focus on their design for the raminder of
this section.
%At the end of the section, we
%list a series of natural extensions that further improve \xray's robustness and
%extensibility. 


\input{correlation}

\input{placement}

\input{input_matching}

% \subsection{Extensions}
% \label{s:extensions}
% We next describe several promising extensions for \xray:
% \heading{Targeting using input combination.}
% For clarity, we have focused on the case where outputs are triggered by a
% \emph{single} input. But the elements of the correlation engine can be extended
% to deal with more general targeting functions, such as input combination defined
% in Appendix~\ref{s:functionmodel}; Thm~\ref{res:placement} indeed is directly
% proved in the general case.

% \iffalse
% \heading{Windowed Tracking.}
% One challenge is dealing with ever-growing input, such as a growing inbox.
% Would one need to continuously create shadow accounts?  Our informal experience
% with Gmail ads suggests that the strength of targeting decreases over time: newer
% emails are targeted more than older ones.  \xray could be extended to track a
% sliding window of inputs, such as the last month's emails.  This would reduce
% the number of shadow accounts required the logarithmic of the number of inputs
% in each window.  If the velocity of a user's inbox is roughly constant, then
% number of shadow accounts should also remain constant over time.
% \fi

% \heading{Collaborative Auditing.}
% One could leverage the input matching scheme to build a collaborative
% auditing scheme, whereby users leverage each others' real
% accounts in lieu of shadow accounts. By contextually matching one user's inputs with those of
% other users, a collaborative \xray might be able to draw sufficient
% differential signal from those users' accounts to uncover behavioral targeting.
% Users would need to share only their emails' signatures with each other or with
% a semi-trusted \xray service, {\em not} the actual content. A hybrid solution
% might also be developed, whereby collaborative filtering is used in cases that
% are not clearly resolved with a small budget of shadow accounts.
% In \S\ref{s:security_analysis} we discuss how this extension could promote
% \xray's robustness to malicious attackers.
%This direction is similar to collaborative spam filtering~\cite{Ramachandran:2007ccs}.




==> functionalanalysis.tex <==
The targeting is specified by the advertisers to the web service.
%, can be modeled as a function taking values $\{0;1\}$ on subsets of inputs. 
%We first treated the case where this value depends on the presence of a single (but unknown) input. 
Appendix~\ref{s:functionmodel} presents a model allowing advertisers to target multiple but finite combinations. We show in Appendix~\ref{s:correctnessproof} that \xray successfully identifies such targeting, again using a \emph{logarithmic} number of accounts.

This model assumes that web services follow a few axiomatic constraints that limits the advertisers' targeting power: (1) targeting campaigns should be \emph{monotone}: this fails only if, \eg Google allows one to target accounts because they did \emph{not} have a specific input, (2) targeting campaigns have a \emph{finite} lists of conditions defining relevant combinations of inputs: this is generally limited by the interface.

An advertiser may attempt to hide by running multiple targeted campaigns using the same adtext, URLs, or even messages. This creates a compound campaigns that can detected as such. Note that this also defeats advertisers' intent to discriminate.

%Note that \xray proves effective targeting on inputs, but not necessarily the intention of the advertisers. 

%How does one track ALL data related to some email?  Maybe I've starred an email in my inbox, what if I don't star it in my shadows?

%Correlation does not mean causation, and when drawing conclusions auditors must be careful about this differentiation.  For example, XXX Nick's point page 18.  Once a problem has been identified, a deep investigation must be performed~\cite{Diakopoulos:2014wo}.





==> placementproof.tex <==
\section{Properties of targeting functions}
\label{s:functionmodel}

Before we prove our main result on the invertibility of targeting functions, we need to describe the properties they satisfy, starting with a few general definitions.

\subsection{How to represent targeting functions?}

\paragraph{Combination, targeting function}
In the following we assume that we have $n$ inputs to start with. Usually we will be interested later to understand how to deal with the case where $n$ is getting large. 

\newcommand{\comb}{\mathcal{C}}
\begin{itemize}
\item 
	An input \emph{combination} $\comb$ of order $r$, sometimes called $r$\_combination is a subset of $r$ distinct elements among the $n$ input. 
\end{itemize}
Note that a $1$\_combination is simply a singleton containing one input.
Intuitively, the word combination will be used in a context where the presence of \emph{all} these inputs together is responsible for some targeting. 

For a given ad, its associated \emph{targeting function} is a mapping $f$ from any combination of inputs into $\{0,1\}$, where $1$ denotes here that an account containing this subset of inputs should be targeted. By convention, untargeted ads are associated with the null function $f(.)=0$. 

We expect that $f$ satisfies these natural axioms:
\begin{itemize}
	\item%($i$)
		\textbf{monotonicity}: $\comb\subseteq \comb' \implies f(\comb)\leq f(\comb')$. 
	\item%($ii$)
		\textbf{input-sensitivity}: $\exists S \midwor{such that} f(\comb)=0$.
\end{itemize}
Monotonicity simply reflects that an account with strictly more interest or hobbies should in theory be relevant to more ads, and never to less. Input sensitivity is only here to avoid the degenerate case where a targeting function makes no discrimination.

\paragraph{Family, explaining relation}
We consider combination as opposed to only single inputs because it might be important for a targeting function to distinguish that multiple inputs occurs simultaneously. Occasionally, it is also the case that different inputs both lead to the same targeting. We capture both using a refined notion:
\begin{itemize}
\item 
	A \emph{family} $S$ of size $l$ is any collection of $l$ distincts combinations. The order of this family is the largest order of any combination it contains. 
\end{itemize}
	For example, a family of order $1$ and of size $l$ is a collection of $l$ different singletons, which hence contains each one different element chosen among the $n$ inputs. 

The following order relation will play a key role in our inference result.
\begin{itemize}
\item 
	We say that a family $S$ \emph{explains} another $S'$ if for any combination $\comb'$ in $S'$ there exists a combination $\comb\in S$ such that $\comb\subseteq\comb'$.
\end{itemize}

For example, with $n=4$ inputs, 
$S=\lset\{1,3\}\vf \{4\}\rset$ and 
$S'=\lset \{1,2,3\}\vf \{4\}\vf \{2,4\}\vf \{1,3\}\rset$ 
we see that $S$ explains $S'$. 
Intuitively, if $S$ explains $S'$, then if we were to observe that all combinations in $S'$ receive an ad, this could in theory be explained by the hypothesis that the ad is targeted at account which contains any of the combination of inputs in $S$. Alternatively, if $S$ does not explain $S'$, then it shows that $S$ is not sufficient on its own to interpret this observation.

According to these definitions, a family $S$ of size $1$ contains a single combination $\comb$. It explains another $S'$ if all combination of inputs in $S'$ are superset of $\comb$. To take another example, a family $S$ of order $1$ is a collection of singletons. It explains another family $S'$ if and only if all combination in $S'$ include each at least one elements in a singleton of $S$. 

\paragraph{Relation between targeting functions and families}
There are many ways to connect targeting functions and families. One can consider the family of subset of inputs that the targeting functions considered relevant $S_{f} = \lset \comb \dimset f(\comb)=1\rset$, and in fact, this family characterizes entirely $f$. Note that, unless $f$ is identically equal to $0$, $f(\{1,\ldots,n\})=1$ and, hence, $S_{f}$ has order $n$ which is maximum and does not depend on $f$. 

\begin{itemize}
	\item We say that a family $S$ \emph{explains} $f$ if and only if $S\subseteq S_f$ and $S$ explains $S_{f}$. 
\end{itemize}
In other words, a family $S$ explains $f$ if all its combination are relevant, and for any combination that $f$ finds relevant, at least one combination in $S$. Interestingly, while $S_f$ have order $n$ unless $f$ is null, a family $S$ that explains $f$ may be much smaller in size and order. For example, if all subsets that are relevant contain one particular input $i$, the the function $f$ is explained by the singleton $i$.

\subsection{The complexity of targeting functions?}

Our goal is to define a black box test and algorithm that detect which input explains targeting with only a small number of tests as $n$ grows large.
So far, we have only assumed that targeting function are monotone and input sensitive. It remains too broad, and the space of such functions is too large to reconstruct any of them from a small number of tests only. One can build intricate worst case counter examples of functions that are hard to revert because they only differ only when many inputs are present. 

Also, this space looks too general to capture the expected behavior of a real targeting function. For example, in the case of an advertiser, the choice of targeting is given through a few $\texttt{or}$, $\texttt{and}$ operators applied to the input. There are also good practical reasons to limit how much of these operators are used. Specifying too much $\texttt{and}$ in the definition of a target may be too narrow: It reduces the population of users concerned potentially below any level that yields effective advertising results (i.e. the intersection of people who lives in New York, expressed an interest in biking, have small kids and are looking for a job may simply be too small for a company to bother). Similarly, specifying too many $\texttt{or}$ operations makes it difficult to build a consistent advertising message (i.e. the union of people who have any of the traits above may have nothing in common with any specific products). 

We now introduce two axioms that intuitively limits how many of these operations are used to define a target, and explains the behavior we observe. 

The first axioms is formally defined as:
\begin{itemize}
	\item 
	\textbf{finite explanation:} We say that $f$ is $l$\_explainable if there exists a family $S$ of size $l$ that explains $f$. 
\end{itemize}
According to this axiom, there exists a small ``core'' family $S$ such that all inputs that leads to targeting are exactly those who include at least one combination chosen in $S$ inside them. For example, if $f\left( \comb \right)$ takes value $1$ exactly when $\comb$ contains either $\{1,3\}$ or $\{4,2\}$ as a subset, then it is $2$\_explainable. A function $f$ that is $1$\_explainable is one that simply checks whether the combination contains one particular combination of input. Hence the value of $l$ loosely represents how many \texttt{or} operations are used to define $f$, or equivalently how many combinations of inputs are considered relevant.

While the first axiom bounds the \emph{number} of combinations that are considered to be targeted, the second axiom defined below bounds the \emph{length} of each combination. It is hence essentially playing the same role for the $\texttt{and}$ operation. 
\begin{itemize}
	\item%($iii$) 
		\textbf{finite order:} We say that $f$ is of \emph{order} $r$ if it is explained by a family $S$ or order $r$. 
\end{itemize}
Remember that, unless $f$ is null, $S^{(f)}$ has order $n$. By monotonicity, the function $f$ will consider the combination of all inputs as ``relevant''. On the other hand, if a family $S$ with order $r$ explains $f$, then what it actually means is that the combination of inputs that were used to decide are much smaller.

A less compact but more illustrative definition is as follows: for any monotone targeting function $f$, let us define $f^{(r)}: \comb \mapsto\max\left( f(\comb') \right.\left| \comb'\subseteq \comb\vf |\comb'|\leq r \right)$. One can easily see that we always have $f\geq f^{(r)}$ and the two functions are so called \emph{$r$\_equivalent}, a notion we define for two functions that coincide for any input combination of order at most $r$. The function $f^{(r)}$ is of order $r$ as it is explained by the family $S^{(r)}_{f} = \lset \comb \dimset f(\comb)=1 \midwor{and} |\comb|\leq r\rset$. In other words, this function considers values of $f$ on all combination of order up to $r$ and then extends the value by monotonicity only. In particular, it does not actively look for a longer combination to decide to return 1. 

\begin{lem}
	The following conditions are equivalent:
	%\begin{itemize}
	(i)~$f$ is of order $r$; (ii)~$f^{r}=f$; (iii)~$S^{(r)}_f$ explains $S_f$; (iv)~the function $f$ is minimal in its $r$\_equivalent class. 
	%\end{itemize}
\end{lem}

\begin{proof}
	Assertion \emph{(iv)} implies \emph{(ii)} that implies \emph{(iii)} that implies \emph{(i)} according to property of $f^{(r)}$ mentioned above. Assertion \emph{(i)} implies \emph{(iv)} as follows: if $f$ is of order $r$ and $g$ is $r$\_equivalent to $f$, it suffices to show that $f(\comb)=1 \implies g(\comb)=1$ to conclude. Since $\comb\in S_f$, we know there exists $\comb'$ or order at most $r$ such that $f(\comb')=1$ and $\comb'\subseteq\comb$. By monotonicity, $g(\comb)\geq g^{(r)}(\comb) \geq g^{(r)}(\comb') = f^{(r)}(\comb')=f(\comb')=1$, which proves the result.
\end{proof}

\paragraph{Core explaining family}
To conclude, we show that any targeting functions which satisfy all our axioms will be associated with a unique family of inputs that explains this targeting the best.

\begin{lem}
	A monotone, input-sensitive targeting function satisfies finite explanation and has finite order if and only if there exists a unique family $S$ satisfying:
	\begin{itemize}
		\item[($i$)] $S$ has size $l$ and order $r$.
		\item[($ii$)] No family of size $l'<l$ explains $f$.
		\item[($iii$)] No family of order $r'<r$ explains $f$.
	\end{itemize}
\end{lem}

\begin{proof}
	When such a family exists, the targeting function is by definition $l$\_explanainable and of order $r$. To show the converse, we know the function admits one explaining family $S_1$ of minimum size $l$ and one $S_2$ of minimum order $r$. We need to construct an explaining family that satisfies both conditions at the same time. Here is how: Since $S_1\subseteq S_f$ and $S_2$ explains $S_f$, then $S_2$ explains $S_1$. In fact, we can associate with each combination $\comb$ in $S_1$ one chosen in $S_2$ that is contained in $\comb$, and hence we create a new family $S$. We claim it has all these properties.

	First, since $S$ is composed of elements in $S_2$ its order it at most $r$. Second, since $S$ contains one combination for each elements in $S_1$ it has at most $l$ combination. Finally, by construction $S$ explains $S_2$, which by transitivity implies that it explains $S_f$, and hence since it is also contained in it, it explains $f$.

	$S$ satisfies all conditions, for minimum value of $l$ and $r$. It only remains to show that it is unique. If another $S'$ family had the same property, we could deduce that $S$ explains $S'$ and vice versa. One can see that any element of $S'$ would be associated with one in $S$ in a one to one mapping. Since they cannot all be equal, it implies that one is strict contained in the other. But the same argument works in the other direction that would lead to a contradiction.
\end{proof}

We define this unique family that explains targeting with minimum information as the \emph{core} explaining family.

\section{Correctness of random input placement}

\label{s:correctnessproof}

Equipped with the definition of targeting function we can now formulate and prove our most general result. The following theorem shows that an algorithm that uses a \emph{logarithmic} amounts of accounts is still able to correctly identify the inputs responsible for targeting, even whey they overlap and are used in combination.

\begin{thm}
	We assuming $\pin,\punt$ are fixed, $\pout$=0. We assume the targeting functions satisfy our four axioms (monotonicity, input sensitivity, finite explaination and finite order). Moreover, we assume that as $N$ grows, the order and size of the functions stay bounded.  
	We introduce $\varepsilon>0$ arbitrarily small. 
	
	There exists an algorithm using $C\times \ln(N)$ accounts which correctly identifies for each ad the core explaining family of the targeting function with probability $(1-\varepsilon)$.
\end{thm}

For clarity, we will first develop the proof when the targeting function is of order $1$, but possibly of any size (the case of \texttt{or} operation). We then provide the proof when the targeting function used is of any order and size $1$ (the case of \texttt{and} operation). The combined proof that generalizes it to simultaneously any order and any size is shown after. This last argument is a bit more involved, since a few recursion steps are used to deal with the way intersecting sets are nested.

\subsection{Property of Bernouilli Family}

Let us start with a few definitions
\begin{itemize}
	\item 
		A random \emph{Bernoulli subset}, denoted by $B(n,p)$ is a subset such that any of $n$ elements is contained with probability $p$ independently of all others.
\item 
	A random \emph{Bernoulli family} of size $m$ is a collection of $m$ independent Bernouilli subsets.
\end{itemize}

The main technical we need for the proof is to show that there does not exists an element or a subset that we encounter in \emph{all} subsets of a Bernouilli family, as long as the family contains a number of subsets that gros logarithmically in $n$. This intuitively shows that if we are given a set of inputs that have been targeted, they may contain one input in common only if that input was relevant to the targeting, and not by mere chance.

\begin{lem}
	Consider a sequence of independent Bernouilli subsets $B_1(n,p),B_2(n,p),\ldots$ and assume there exists $C>(\ln(\frac{1}{p}))^{-1}$ such that $m=C\cdot \ln(n)$, then the event $B_1(n,p)\cap\ldots\cap B_m(n,p)=\emptyset$ is almost sure as $n$ goes large.
\end{lem}

\begin{proof}
	We first observe that:
	\[
	\begin{disarray}[c]{c}
	\lset B_1(n,p)\cap\ldots\cap B_m(n,p) =\emptyset\rset \\
	= \bigcap_{i=1}^n \lset i\notin B_1(n,p)\cap\ldots\cap B_m(n,p) \rset \ff
	\end{disarray}
	\]
	This directly implies that 
	\[
	\begin{disarray}[c]{c}
	\probaof{B_1(n,p)\cap\ldots\cap B_m(n,p) =\emptyset} 
	= \prod_{i=1}^n \left( 1-p^m \right) \\
	= \left( 1-p^m \right)^{n} 
	= e^{n\cdot \ln(1-p^m)}
	\ff
	\end{disarray}
	\]
	The probability of this event converges to $1$ if and only if $n\cdot \ln(1-p^m)$ goes to $0$ as $n$ grows. 
	
	Assuming $m=C \cdot\ln(n)$ (where the value of $C$ can be chosen arbitrarily) the later expression may be rewritten $n\cdot \ln(1-n^{-C\ln(\frac{1}{p})})\sim_{n\to\infty} n^{1-C\ln(\frac{1}{p})}$ as $n$ goes large, which proves the lemma. 
\end{proof}

The result above is sufficient to determine the \emph{core} explaining family of a targeting function as long one know that it contains a single combination. In fact, in such situation, this combination will be present in \emph{all} targeted accounts. The lemma above proves that when it is the case, it cannot be attributed to chance. 

On the other hand, when multiple combinations could be triggering a targeting function, then this argument fails, and we need a stronger bound to exclude that we find a core explaining family by chance. 

Let $S$ be any subset, we say it \emph{intersects} a family if for any subset $B$ in the family, we have $S\cap B\neq \emptyset$. Note that a family admits an intersection subset of size $1$ if and only if its intersection is nonempty. On the other hand, even family that have a null intersection may admit intersecting subsets of larger size.

\begin{lem}
	Consider a Bernouilli family of size $m=C\cdot \ln(N)$, where 
	$C>l / \ln\left( \frac{1}{1-(1-p)^l} \right)$ 
	then, almost surely, as $N$ goes large, there does not exist an intersecting subset of size at most $l$.
\end{lem}

\begin{proof}
	Since the constant $C$ only increases with $l$ by recurrence it suffices to show that the result holds for subset of size exactly $l$. For a given subset $S$ of size $l$, any single Bernouilli subset will intersect it with probability $1-(1-p)^{l}$. Hence this subset intersects a family of $m$ such independent subsets with a probability $(1-(1-p)^{l})^{m}$. With $n \choose l$ possible subsets, the probability that they all fail to intersects the family is
	\[
	\Delta^{(l)}(m,n) = \left( 1-(1-(1-p)^{l})^{m} \right)^{n\choose l}
	\ff
	\]
	After taking the logarithm, one obtains
	\[
	\begin{disarray}[c]{c}
		\ln (\Delta^{(l)}(m,n))  = {n\choose l}
		\ln \left( 1-(1-(1-p)^{l})^{m} \right) \\
		 \sim \frac{n^l}{l!} (1-(1-p)^{l})^{m} \\
		 \sim \frac{1}{l!} \exp
		 \left( 		 l\cdot \ln(n) -m\cdot \ln\left( \frac{1}{1-(1-p)^{l}} \right)  \right)\ff
\\
	\end{disarray}
	\]
	Which proves the result since assuming $m$ grows as $\ln(n)$ with a strictly larger constant would make the difference in the exponential going to $-\infty$ as $n$ goes large, which would imply that $\ln(\Delta^{(l)}(n,p))$ goes to $0$ which implies that the probability $\Delta^{(l)}(n,p)$ goes to 1.	
\end{proof}

The results above is much stronger: It proves that if a small subset of up to $l$ inputs are found in all the accounts that have been targeted, this cannot be an effect of chance.

We are now equipped to prove our main results.

\subsection{Targeting on a single combination}

In this case, we assume that the core explaining family has size $1$: In other words, the targeting function $f$ only tests the inputs of the account in that it return $1$ if a particular (unknown) combination is found. After running our random placement algorithm on $C\times \ln(N)$ accounts, at least an expected $C \alpha^r \ln(N)$ accounts contain this combination, and since we target any account with the combination with probability $\pin$, we obtain in expectation $C\alpha^r\pin\ln(N)$ accounts that are targeted. Using Chernoff bound, we can even prove that we obtain with very high probability a number of account that are of the order of this expectation. 

By definition, the combination will be found in all targeted accounts, but it may be that by chance, these accounts also contains collectively another of the $N-r$ inputs that was included merely by chance.  Assuming $C$ is properly chosen, we know that with probability $1$ as $N$ goes large, this cannot happen: Since the remaining inputs chosen in the $N-r$ constitutes a Bernouilli family, it has an empty intersection as soon as the number of account is sufficiently large.

This completes the proof, since we show that when targeting occurs, the targeted combination is always the intersection of inputs for all targeted accounts with high probability. Note that if the ad was not targeted, exactly the same reasoning will prove that this intersection is empty.

\subsection{Targeting of a family of combination of order $1$}

We now deal with a much more difficult case in which multiple combinations (up to $l$ of them) can each trigger the ad for which the targeting function is to be inverted. In this situation, one combinations that is responsible for some of the targeted ads is \emph{not} in general found in all targeted accounts. This renders the argument used above entirely ineffective. A naive algorithm based on intersection only could conclude that no targeting too place, since the intersection is null. Even worse, it might incorrectly conclude that the ads are targeted by a single input, which is in fact common to 2 combinations that are targeted.

We treat the case in which all combinations that are targeted are of order $1$. In other words, a subset of the input of size at most $l$ is such that an account that contains any of them is targeted.

Our algorithm works as follows: After a random placement of inputs into $C\times \ln(N)$ accounts, the algorithm consider all the accounts that have been targeted. It then looks for a subset of minimum size that intersects the inputs of all these targeted accounts. Since we assume that targeted account never occurs out of mistake (\ie $\pout=0$), we know that it will necessarily find a subset containing at most $l$ inputs that intersects all of these. In fact, since we have a growing number of account, and a constant probability to include any inputs and consecutively be targeted for it, all inputs will appear in this set. The only remaining question is whether additional inputs could be present in sufficient account that they pollute this set. 

Like above, an application of our analysis of Bernouilli family can convince us that this cannot be the case. Assuming first that the ad is untargeted, inputs in accounts seeing the ads are a Bernouilli family of logarithmic size. We have already seen that for a fixed $l$ such family do not admit an intersecting subset of size up to $l$. Our algorithms hence answers correctly with high probability. If on the contrary this ad is targeted towards any email in a particular subset of size $l$, an element of this targeted subset will be present in each targeted account, but since all other elements appear as part of a Bernouilli subset, they are not susceptible to form any intersecting subsets, or even to pollute it. It would otherwise prove that a positive probability exists for an intersecting subset of size less than $l$ to form within randomly placement element, which would contradict our lemma.

\subsection{Targeting in the most general case}

When targeting is made on an arbitrary number $l$ of combination up to arbitrary length $r$, the same result holds but the algorithm and the proof is slightly more complicated. It works with exactly the same placement (a random $C\times\ln(N)$ of inputs are included in each account), in a recursive manner, with up to $l$ phase:

In the first step, the algorithms looks for the smallest intersecting subset with inputs seen in targeted accounts. If the ad is untargeted, it would not have a small intersecting set (less than $l$) with large probability, and it would be sufficient to detect that. If it is targeted, then we are choosing the set of emails as ``candidates'' to be targeted.

The difficulty comes from the following fact: how would the algorithm detects the difference between a targeting function looking for the combination $\{1,3\}$ and $\{1,4\}$ and a targeting function that looks for $\{1\}$. In the first phase, $1$ would be a candidate since it is seen in all accounts. So far, our algorithm cannot distinguish them. 

In the second phase, we apply recursively our algorithm by restricting to all accounts that contains a candidate. If this email is actually the one that is used, then using a similar argument, there should not be any intersecting subsets within this account. In other words, email will appear untargeted \emph{within this set}, we hence apply our algorithm in this case, and would conclude that the ``candidate'' is actually the one targeted. Otherwise, if there exists a small intersecting subset of inputs, then it means that some higher order combination are the one responsible for the targeting. They create each candidates of order $2$ (in which the original candidate and one element in the new intersecting subset will appear). 

We can then apply recursively the algorithm to each of these order $2$ candidates, and stop whenever the ``remaining'' accounts do not appear to have a small intersecting subset. If $C$ is chosen large enough, then even after possibly $r$ steps of recursion there is still a logarithmic number of accounts, which allows all the same arguments to hold.


